DoCoFL: Downlink Compression for Cross-Device Federated Learning

Many compression techniques have been proposed to reduce the communication overhead of Federated Learning training procedures. However, these are typically designed for compressing model updates, which are expected to decay throughout training. As a result, such methods are inapplicable to downlink (i.e., from the parameter server to clients) compression in the cross-device setting, where heterogeneous clients $\textit{may appear only once}$ during training and thus must download the model parameters. Accordingly, we propose $\textsf{DoCoFL}$ -- a new framework for downlink compression in the cross-device setting. Importantly, $\textsf{DoCoFL}$ can be seamlessly combined with many uplink compression schemes, rendering it suitable for bi-directional compression. Through extensive evaluation, we show that $\textsf{DoCoFL}$ offers significant bi-directional bandwidth reduction while achieving competitive accuracy to that of a baseline without any compression.

==> sections/main_proof.tex <==
We prove convergence for a more general framework where each client can use any model up to $\Tcal$ rounds prior to the current round. 

\begin{algorithm}
\caption{\methodName}\label{alg:distributed_SGD}
% \DontPrintSemicolon
% \KwInput{Learning rate $\eta$;
% Global/local learning rates $\eta_g, \eta_{\ell}$;
\begin{algorithmic}
    \STATE {\bfseries Input:} Initial weights $x_0\in\reals^d$
    \FOR{$t=0,\ldots,T-1$}
        \STATE Randomly sample a subset of $S$ clients, $\Scal_{t}\subseteq\sbrac{N}$
        \FOR{client $i\in\Scal_{t}$ in parallel}
            \STATE Obtain model weights, $y_t^i = x_{t - \tau_t^i}$ $\hspace{9.4cm}\triangleright$ $\tau_t^i\in\sbrac{0, \Tcal}$
            \STATE Obtain compressed correction,
            $\hat{\Delta}_{t}^i = \C(x_t - y_t^i)$
            \STATE Construct model estimate, $\hat{x}_t^i = y_t^i + \hat{\Delta}_t^i$
            \STATE Compute local gradient, $\hat{g}_t^i = g_t^i(\hat{x}_t^i)$
            \STATE Communicate $\hat{g}_t^i$ back to server
        \ENDFOR
        % \tcc{On server}
        \STATE Aggregate local gradients, $\hat{g}_t\coloneqq \frac{1}{S}\sum_{i\in\Scal_t}{\hat{g}_{t}^{i}}$
        % Aggregate: $\Delta_{r}^{(0)} = \frac{1}{S}\sum_{i\in\Scal_{r}^{(0)}}{\Delta_{i}^{(r,0)}}$\\
        \STATE Update iterate, $x_{t+1} = x_{t} - \eta \hat{g}_t$
    \ENDFOR
    % \STATE {\bfseries Output:} $x_s\sim\text{Uniform}(x_1,\ldots, x_T)$
\end{algorithmic}
\end{algorithm}

For the ease of notation, let $\nab_t\coloneqq \nabla f(x_t)$. We start with establishing a bound on the second moment of the aggregated gradient $\hat{g}_t$. 
\begin{Lem}\label{lem:second_moment_bound}
    Suppose Assumptions~\ref{assump:bounded_variance}, \ref{assump:bgd}, and~\ref{assump:bounded_nmse} hold. Then, for every $t\in\sbrac{T}$, it holds that
    \begin{equation}
        \bbE\norm{\hat{g}_t}^2 \leq \tilde{\sigma}^2 + 4\gamma\bbE\norm{\nab_t}^2 + 2\beta^2\cdot\frac{1}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2}\; ,
    \end{equation}
    where $\tilde{\sigma}^2\coloneqq \frac{\sigma^2}{S} + \brac{1 - \frac{S}{N}}\frac{4G^2}{S}$ and $\gamma\coloneqq 1 + \brac{1 - \frac{S}{N}}\frac{B^2}{S}$.
\end{Lem}
\begin{proof}
    Since $\hat{g}_t$ is an aggregation of local gradient, we can write,  
    \begin{align}
        \bbE\norm{\hat{g}_t}^2 &= \bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\hat{g}_t^i}}^2 = \bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\brac{\hat{g}_t^i - \nabla f_i(\hat{x}_t^i) + \nabla f_i(\hat{x}_t^i)}}}^2 \nonumber \\ &= \bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\brac{\hat{g}_t^i - \nabla f_i(\hat{x}_t^i)}}}^2 + \bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\nabla f_i(\hat{x}_t^i)}}^2 \nonumber\; ,
    \end{align}
    where the last equality follows from Assumption~\ref{assump:bounded_variance} as $\bbE[(\hat{g}_t^i(\hat{x}_t^i) - \nabla f_i(\hat{x}_t^i))^\top \nabla f_i(\hat{x}_t^i)] = 0$. Note that the first term in the right-hand side is the variance of the average of $S$ independent random variables with zero mean and variance bounded by $\sigma^2$; therefore, it is bounded by $\sigma^2/S$. Thus, we get that
    \begin{equation}\label{eq:main_proof_second_moment}
        \bbE\norm{\hat{g}_t}^2 \leq \frac{\sigma^2}{S} + \bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\nabla f_i(\hat{x}_t^i)}}^2\; .
    \end{equation}
    Focusing on the second term in the right-hand side, we have that
    \begin{equation}
        \bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\nabla f_i(\hat{x}_t^i)}}^2 \leq \underbrace{2\bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\brac{\nabla f_i(\hat{x}_t^i) - \nabla f_i(x_t)}}}^2}_{(A)} + \underbrace{2\bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\nabla f_i(x_t)}}^2}_{=(B)}\; ,
    \end{equation}
    where we used the inequality $\norm{a + b}^2 \leq 2\norm{a}^2 + 2\norm{b}^2$.

    \paragraph{Bounding $(A)$: } Using Lemma~\ref{lem:technical_norm_of_sum_to_sum_of_norms} and the $\beta$-smoothness of the objective, we get that 
    \begin{align}
        2\bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\brac{\nabla f_i(\hat{x}_t^i) - \nabla f_i(x_t)}}}^2 &\leq \frac{2}{S}\bbE\sbrac{\sum_{i\in\Scal_t}{\norm{\nabla f_i(\hat{x}_t^i) - \nabla f_i(x_t)}^2}} \nonumber \\ &\leq \frac{2\beta^2}{S}\bbE\sbrac{\sum_{i\in\Scal_t}{\norm{\hat{x}_t^i - x_t}^2}} \nonumber \\ &= \frac{2\beta^2}{S}\bbE\sbrac{\sum_{i=1}^{N}{\norm{\hat{x}_t^i - x_t}^2}\cdot\mathbbm{1}_{\cbrac{i\in\Scal_t}}}\nonumber\\ &= \frac{2\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2} \nonumber\; ,
    \end{align}
    where the last equality holds because sampling the subset of clients $\Scal_t\subseteq\sbrac{N}$ is independent of the optimization process, and $\prob(i\in\Scal_t) = S/N$.   

    \paragraph{Bounding $(B)$: } By the law of total expectation, $(B)$ can be written as follows,
    \begin{equation}\label{eq:main_proof_bounding_B}
        2\bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\nabla f_i(x_t)}}^2 = 2\bbE\bnorm{\sum_{i=1}^{N}{\brac{\frac{1}{S}\nabla f_i(x_t)\cdot\mathbbm{1}_{\cbrac{i\in\Scal_t}}}}}^2 = 2\bbE\sbrac{\bbE\sbrac{\bnorm{\sum_{i=1}^{N}{\brac{\frac{1}{S}\nabla f_i(x_t)\cdot\mathbbm{1}_{\cbrac{i\in\Scal_t}}}}}^2~\vrule~x_t}}\; .
    \end{equation}
    Thus, we can use Lemma~\ref{lem:technical_norm_of_sum_of_iid} with $X_i = \frac{1}{S}\nabla f_i(x_t)\cdot\mathbbm{1}_{\cbrac{i\in\Scal_t}},~ i\in\sbrac{N}$ to bound the inner expectation. Using $\prob(i\in\Scal_t) = S/N$, we have that
    \begin{equation*}
        \bbE[X_i|x_t] = \frac{1}{S}\nabla f_i(x_t)\cdot\frac{S}{N} = \frac{1}{N}\nabla f_i(x_t), 
    \end{equation*}
    and, 
    \begin{align*}
        \bbE[\norm{X_i - \bbE[X_i|x_t]}^2|x_t] &= \norm{\nabla f_i(x_t)}^2 \cdot\bbE\sbrac{\brac{\frac{1}{S}\cdot\mathbbm{1_{\cbrac{i\in\Scal_t}}} - \frac{1}{N}}^2} =  \norm{\nabla f(x_t)}^2\cdot\text{Var}\brac{\frac{1}{S}\cdot\mathbbm{1}_{\cbrac{i\in\Scal_t}}} \\ &=  \frac{\norm{\nabla f(x_t)}^2}{S^2}\cdot \frac{S}{N}\brac{1 - \frac{S}{N}} = \frac{\norm{\nabla f_i(x_t)}^2}{SN}\brac{1 - \frac{S}{N}}\; ,
    \end{align*}
    where we used the fact that for any event $\A$, the following holds: $\text{Var}(\mathbbm{1}_{\A}) = \prob(\A)\cdot(1 - \prob(\A))$. Therefore, using Lemma~\ref{lem:technical_norm_of_sum_of_iid}, we obtain that 
    \begin{align*}
        \bbE\sbrac{\bnorm{\sum_{i=1}^{N}{\brac{\frac{1}{S}\nabla f_i(x_t)\cdot\mathbbm{1}_{\cbrac{i\in\Scal_t}}}}}^2~\vrule~x_t} &\leq 2\bnorm{\frac{1}{N}\sum_{i=1}^{N}{\nabla f_i(x_t)}}^2 + \frac{2}{SN}\brac{1 - \frac{S}{N}}\sum_{i=1}^{N}{\norm{\nabla f_i(x_t)}^2} \\ &\leq 2\norm{\nab_t}^2 + \frac{2}{S}\brac{1-\frac{S}{N}}\brac{G^2 + B^2\norm{\nab_t}^2} \\ &= \brac{1 - \frac{S}{N}}\frac{2G^2}{S} + 2\underbrace{\brac{1 + \brac{1 - \frac{S}{N}}\frac{B^2}{S}}}_{\coloneqq\gamma}\norm{\nab_t}^2 \; ,
    \end{align*}
    where in the second inequality we used the bounded gradient dissimilarity assumption (Assumption~\ref{assump:bgd}). Plugging back to Eq.~\eqref{eq:main_proof_bounding_B}, we get the following bound on $(B)$:
    \begin{equation*}
        2\bbE\bnorm{\frac{1}{S}\sum_{i\in\Scal_t}{\nabla f_i(x_t)}}^2 \leq \brac{1 - \frac{S}{N}}\frac{4G^2}{S} + 4\gamma\bbE\norm{\nab_t}^2\; .
    \end{equation*}
    
    Plugging the bounds on $(A)$ and $(B)$ in Eq.~\eqref{eq:main_proof_second_moment} finally gives
    \begin{align*}
        \bbE\norm{\hat{g}_t}^2 &\leq \frac{\sigma^2}{S} + \brac{1 - \frac{S}{N}}\frac{4G^2}{S} + 4\gamma\bbE\norm{\nab_t}^2 + \frac{2\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2} \\ &= \tilde{\sigma}^2 + 4\gamma\bbE\norm{\nab_t}^2 + \frac{2\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2}\; ,
    \end{align*}
    which concludes the proof. 
\end{proof}

The next result establishes a bound on the model estimation error of the clients.
\begin{Lem}\label{lem:model_estimation_error}
    Let $\alpha\coloneqq \beta^2\omega^2\Tcal^2\eta^2$, and $\nabla_{-\ell}\coloneqq 0, \enskip\forall \ell\in\naturals$. Then, the following result holds:
    \begin{equation*}
        2\beta^2 \bbE\norm{\hat{x}_t^i - x_t}^2 \leq \sum_{k=1}^{t}{k (2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{t}{(2\alpha)^k\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}\; .
    \end{equation*}
\end{Lem}

\begin{proof}
    We prove this lemma using strong induction. For the base case, we show that the result holds for any $t=0,\ldots,\Tcal$. Then, we assume that the result holds for any $s=t-\Tcal,\ldots,t-1$, and show that it also holds for $s=t$. 
    
    We start with some general observations that hold for any $t$.  Recall that $\hat{x}_t^i = y_{t}^i + 
    \C(x_t - y_t^i)$. From Assumption~\ref{assump:bounded_nmse}, we have
    \begin{equation}\label{eq:model_estimation_err}
        \bbE\norm{\hat{x}_t^i - x_t}^2 = \bbE\norm{\C(x_t - y_t^i) - (x_t - y_t^i)}^2 \leq \omega^2\bbE\norm{x_t - y_t^i}^2 \; .
    \end{equation}
    Unrolling the update rule for $x_t$, we have for all $i\in\sbrac{N}$ that 
    \begin{equation*}
        x_{t} = x_{t -\tau_t^i} - \eta\sum_{k=t-\tau_t^i}^{t-1}{\hat{g}_k} = y_t^i - \eta\sum_{k=t-\tau_t^i}^{t-1}{\hat{g}_k} \; .
    \end{equation*}
    Let $\hat{g}_{-k}\coloneqq 0$ for all $k\in\naturals$. Plugging back to Eq.~\eqref{eq:model_estimation_err} and using Lemma~\ref{lem:technical_norm_of_sum_to_sum_of_norms} we get that
    \begin{align}\label{eq:model_estimate_err_sum_of_grads}
        \bbE\norm{\hat{x}_t^i - x_t}^2 &\leq \omega^2\eta^2\bbE\bnorm{\sum_{k=t-\tau_t^i}^{t-1}{\hat{g}_k}}^2 \leq \omega^2\eta^2\tau_t^i\sum_{k=t-\tau_t^i}^{t-1}{\bbE\norm{\hat{g}_k}^2} \leq \omega^2\eta^2\Tcal\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\hat{g}_k}^2} \; ,
    \end{align}
    where the last inequality follows from $\tau_t^i\leq\Tcal$. 
    
    \textbf{Base Case: } For every $t=1,\ldots,\Tcal$ and $i\in\sbrac{N}$, we have from Eq.~\eqref{eq:model_estimate_err_sum_of_grads} that
    \begin{equation}\label{eq:model_estimate_err_base_case}
        \bbE\norm{\hat{x}_t^i - x_t}^2 \leq \omega^2\eta^2\Tcal\sum_{k=0}^{t-1}{\bbE\norm{\hat{g}_k}^2}\; .
    \end{equation}
    For $t=0$, each client obtains the exact model weights, i.e., $\hat{x}_0^i = x_0$, which trivially implies that the above inequality also holds in this case. Multiplying by $2\beta^2$, using Lemma~\ref{lem:second_moment_bound} to bound $\bbE\norm{\hat{g}_k}^2$, and using $\beta^2\omega^2\eta^2\Tcal = \alpha/\Tcal$, we get
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq 2\beta^2\omega^2\eta^2\Tcal\sum_{k=0}^{t-1}{\brac{\tilde{\sigma}^2 + 4\gamma\bbE\norm{\nab_k}^2 + \frac{2\beta^2}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2}}} \\ &= 2\alpha\tilde{\sigma}^2 + \frac{8\alpha\gamma}{\Tcal}\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + \frac{4\alpha\beta^2}{\Tcal}\sum_{k=0}^{t-1}{\frac{1}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2}}\; .
    \end{align*}
    Using Eq.~\eqref{eq:model_estimate_err_base_case}, we can bound for every $k=0,\ldots,t-1$:
    \begin{align*}
        \frac{1}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2} \leq \omega^2\eta^2\Tcal\sum_{\ell=0}^{k-1}{\bbE\norm{\hat{g}_{\ell}}^2}\; .
    \end{align*}
    Plugging back, we get
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 \leq 2\alpha\tilde{\sigma}^2 + \frac{8\alpha\gamma}{\Tcal}\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + 4\alpha\beta^2\omega^2\eta^2\sum_{k=0}^{t-1}{\sum_{\ell=0}^{k-1}{\bbE\norm{\hat{g}_\ell}^2}}\; .
    \end{align*}
    Note that we can bound the double sum in right-hand side using Lemma~\ref{lem:double_sum_to_single_sum} as
    \begin{equation*}
        \sum_{k=0}^{t-1}{\sum_{\ell=0}^{k-1}{\bbE\norm{\hat{g}_\ell}^2}} \leq t\sum_{k=0}^{t-2}{\bbE\norm{\hat{g}_k}^2} \leq \Tcal\sum_{k=0}^{t-2}{\bbE\norm{\hat{g}_k}^2}\; ,
    \end{equation*}
    where the last inequality follows since $t\leq\Tcal$. Plugging this result back gives
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 \leq 2\alpha\tilde{\sigma}^2 + \frac{8\alpha\gamma}{\Tcal}\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + \frac{4\alpha^2}{\Tcal}\sum_{k=0}^{t-2}{\bbE\norm{\hat{g}_k}^2}\; .
    \end{align*}
    Once again, we can bound $\bbE\norm{\hat{g}_k}^2$ using Lemma~\ref{lem:second_moment_bound} to get
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq 2\alpha\tilde{\sigma}^2 + \frac{8\alpha\gamma}{\Tcal}\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + \frac{4\alpha^2}{\Tcal}\sum_{k=0}^{t-2}{\brac{\tilde{\sigma}^2 + 4\gamma\bbE\norm{\nab_k}^2 + \frac{2\beta^2}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2}}} \\ &\leq \brac{2\alpha + 4\alpha^2}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\brac{2\alpha\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + 4\alpha^2\sum_{k=0}^{t-2}{\bbE\norm{\nab_k}^2}} + \frac{8\alpha^2\beta^2}{\Tcal}\sum_{k=0}^{t-2}{\frac{1}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2}}\; .
    \end{align*}
    And using Eq.~\eqref{eq:model_estimate_err_base_case} to bound $\frac{1}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2}$:
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq \brac{2\alpha + 4\alpha^2}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\brac{2\alpha\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + 4\alpha^2\sum_{k=0}^{t-2}{\bbE\norm{\nab_k}^2}} + 8\alpha^2\beta^2\omega^2\eta^2\sum_{k=0}^{t-2}{\sum_{\ell=0}^{k-1}{\bbE\norm{\hat{g}_\ell}^2}} \\ &\leq \brac{2\alpha + 4\alpha^2}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\brac{2\alpha\sum_{k=0}^{t-1}{\bbE\norm{\nab_k}^2} + 4\alpha^2\sum_{k=0}^{t-2}{\bbE\norm{\nab_k}^2}} + \frac{8\alpha^3}{\Tcal}\sum_{k=0}^{t-3}{\bbE\norm{\hat{g}_k}^2}\; ,
    \end{align*}
    where in the last inequality we used Lemma~\ref{lem:double_sum_to_single_sum} and $\beta^2\omega^2\eta^2\Tcal = \alpha/\Tcal$. Repeating this process of alternately applying Lemma~\ref{lem:second_moment_bound} to bound $\bbE\norm{\hat{g}_k}^2$ and using Eq.~\eqref{eq:model_estimate_err_base_case} and Lemma~\ref{lem:double_sum_to_single_sum} gives
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq \sum_{k=1}^{t}{(2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{t}{(2\alpha)^{k}\sum_{\ell=0}^{t-k}{\bbE\norm{\nab_\ell}^2}}\; .
    \end{align*}
    Note that for all $t\leq\Tcal$ and $k\geq 1$, we have $t-k\Tcal\leq 0$. Therefore, since $\nabla_{-\ell}=0$ for all $\ell\in\naturals$, we can equivalently write:
    \begin{align*}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq \sum_{k=1}^{t}{(2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{t}{(2\alpha)^{k}\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}\; .
    \end{align*}
    Finally, using $(2\alpha)^k\leq k(2\alpha)^k$, which holds for any $k\geq 1$, establishes the result for the base case. 

    \textbf{Induction step: } The induction hypothesis is that the following holds:
    \begin{equation}\label{eq:induction_hypothesis}
         2\beta^2 \bbE\norm{\hat{x}_s^i - x_s}^2 \leq \sum_{k=1}^{s}{k (2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{s}{(2\alpha)^k\sum_{\ell=s-k\Tcal}^{s-k}{\bbE\norm{\nab_\ell}^2}}, \quad\forall s=t-\Tcal,\ldots, t-1 \; .
    \end{equation}
    We focus on Eq.~\eqref{eq:model_estimate_err_sum_of_grads}. Multiplying by $2\beta^2$ and using Lemma~\ref{lem:second_moment_bound} to bound $\bbE\norm{\hat{g}_k}^2$, we get
    \begin{align}\label{eq:client_estimation_error}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq 2\beta^2\omega^2\eta^2\Tcal\sum_{k=t-\Tcal}^{t-1}{\brac{\tilde{\sigma}^2 + 4\gamma\bbE\norm{\nab_k}^2 + \frac{2\beta^2}{N}\sum_{j=1}^{N}{\bbE\norm{\hat{x}_k^j - x_k}^2}}} \nonumber \\ &= 2\alpha\tilde{\sigma}^2 + 4\gamma\cdot\frac{2\alpha}{\Tcal}\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2} + \frac{2\alpha}{\Tcal} \underbrace{\sum_{k=t-\Tcal}^{t-1}{\frac{1}{N}\sum_{j=1}^{N}{2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2}}}_{(\dag)}\; .
    \end{align}
    From the induction hypothesis~\eqref{eq:induction_hypothesis}, we can bound $2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2$ for every $k\in\sbrac{t-\Tcal, t-1}$ as follows:
    \begin{equation*}
        2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2 \leq \sum_{\ell=1}^{k}{\ell(2\alpha)^\ell}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{\ell=1}^{k}{(2\alpha)^\ell \sum_{m=k-\ell\Tcal}^{k-\ell}{\bbE\norm{\nab_m}^2}}\; .
    \end{equation*}
    Denote this bound by $B(k)\coloneqq\sum_{\ell=1}^{k}{\ell(2\alpha)^\ell}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{\ell=1}^{k}{(2\alpha)^\ell \sum_{m=k-\ell\Tcal}^{k-\ell}{\bbE\norm{\nab_m}^2}}$, i.e., $2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2\leq B(k)$. Note that $B(k)$ is independent of $j$; thus, the bound also holds for the average over the clients, $\frac{1}{N}\sum_{j=1}^{N}{2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2}\leq B(k)$.
    % \begin{equation*}
    %     \frac{1}{N}\sum_{j=1}^{N}{2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2} \leq \sum_{\ell=1}^{k}{\ell(2\alpha)^\ell}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{\ell=1}^{k}{(2\alpha)^\ell \sum_{m=k-\ell\Tcal}^{k-\ell}{\bbE\norm{\nab_m}^2}}\; .
    % \end{equation*}
    We can therefore bound $(\dag)$ as
    \begin{equation*}
        \sum_{k=t-\Tcal}^{t-1}{\frac{1}{N}\sum_{j=1}^{N}{2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2}} \leq \sum_{k=t-\Tcal}^{t-1}{B(k)} \leq \Tcal B(t-1)\; .
    \end{equation*}
    where the last inequality holds because $B(k)$ is monotonically increasing.
    % \begin{align}
    %     \sum_{k=t-\Tcal}^{t-1}{\frac{1}{N}\sum_{j=1}^{N}{2\beta^2\bbE\norm{\hat{x}_k^j - x_k}^2}} &\leq \sum_{k=t-\Tcal}^{t-1}{\sum_{\ell=1}^{k}{\ell (2\alpha)^\ell}}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=t-\Tcal}^{t-1}{\sum_{\ell=1}^{k}{(2\alpha)^\ell\sum_{m=k-\ell\Tcal}^{k-\ell}{\bbE\norm{\nab_m}^2}}} \nonumber \\ &\leq \Tcal\sum_{\ell=1}^{t-1}{\ell(2\alpha)^\ell}\tilde{\sigma}^2 + 4\gamma\sum_{\ell=1}^{t-1}{(2\alpha)^\ell\sum_{m=t-1-\ell\Tcal}^{t-1-\ell}{\bbE\norm{\nab_m}^2}} \nonumber \; ,
    % \end{align}
    % where the final inequality holds because 
    % \[
    %     \max_{k\in\cbrac{t-\Tcal,\ldots,t-1}}{\sum_{\ell=1}^{k}{\ell(2\alpha)^\ell}}=\sum_{\ell=1}^{t-1}{\ell(2\alpha)^\ell}, 
    % \]
    % and,  
    % \[ 
    %     \max_{k\in\cbrac{t-\Tcal,\ldots,t-1}}{\sum_{\ell=1}^{k}{(2\alpha)^\ell\sum_{m=k-\ell\Tcal}^{k-\ell}{\bbE\norm{\nab_m}^2}}} = \sum_{\ell=1}^{t-1}{(2\alpha)^\ell\sum_{m=t-1-\ell\Tcal}^{t-1-\ell}{\bbE\norm{\nab_m}^2}}\; .
    % \]
    
    Plugging back to Eq.~\eqref{eq:client_estimation_error} and substituting $B(t-1)$ gives
    \begin{align}\label{eq:lem_model_estimation_err}
        2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2 &\leq 2\alpha\tilde{\sigma}^2 + 4\gamma\cdot\frac{2\alpha}{\Tcal}\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2} + \frac{2\alpha}{\Tcal}\cdot\Tcal B(t-1) \nonumber \\ &= 2\alpha\tilde{\sigma}^2 + \frac{8\gamma\alpha}{\Tcal}\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2} + 2\alpha\cdot\brac{\sum_{k=1}^{t-1}{k(2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{t-1}{(2\alpha)^k\sum_{\ell=t-1-k\Tcal}^{t-1-k}{\bbE\norm{\nab_\ell}^2}}} \nonumber \\ &= \underbrace{\brac{2\alpha + \sum_{k=1}^{t-1}{k(2\alpha)^{k+1}}}}_{(A)}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\underbrace{\brac{2\alpha\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2} + \sum_{k=1}^{t-1}{(2\alpha)^{k+1}\sum_{\ell=t-1-k\Tcal}^{t-1-k}{\bbE\norm{\nab_\ell}^2}}}}_{(B)}\; .
    \end{align}
    \paragraph{Bounding $(A)$: } Note that $(A)$ can be bounded as
    \begin{align*}
        2\alpha + \sum_{k=1}^{t-1}{k(2\alpha)^{k+1}} &= 2\alpha + \sum_{k=2}^{t}{(k-1)(2\alpha)^{k}} \leq 2\alpha + \sum_{k=2}^{t}{k(2\alpha)^{k}} = \sum_{k=1}^{t}{k(2\alpha)^{k}}\; .
    \end{align*}
    \paragraph{Bounding $(B)$: } Focusing on the second sum in $(B)$, we have
    \begin{align*}
        \sum_{k=1}^{t-1}{(2\alpha)^{k+1}\sum_{\ell=t-1-k\Tcal}^{t-1-k}{\bbE\norm{\nab_\ell}^2}} &= \sum_{k=2}^{t}{(2\alpha)^{k}\sum_{\ell=t-1-(k-1)\Tcal}^{t-1-(k-1)}{\bbE\norm{\nab_\ell}^2}} \\ &= \sum_{k=2}^{t}{(2\alpha)^{k}\sum_{\ell=t-k\Tcal + \Tcal-1}^{t-k}{\bbE\norm{\nab_\ell}^2}} \\ &\leq \sum_{k=2}^{t}{(2\alpha)^{k}\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}\; , 
    \end{align*}
    where the last inequality holds since $\Tcal-1\geq 0$ and $\bbE\norm{\nab_\ell}^2\geq 0$ for all $\ell$. Adding $2\alpha\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2}$ to both sides, we can therefore bound $(B)$ as 
    \begin{align*}
        2\alpha\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2} + \sum_{k=1}^{t-1}{(2\alpha)^{k+1}\sum_{\ell=t-1-k\Tcal}^{t-1-k}{\bbE\norm{\nab_\ell}^2}} &\leq 2\alpha\sum_{k=t-\Tcal}^{t-1}{\bbE\norm{\nab_k}^2} + \sum_{k=2}^{t}{(2\alpha)^{k}\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}} \\ &= \sum_{k=1}^{t}{(2\alpha)^{k}\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}\; .
    \end{align*}
    
    Plugging back to Eq.~\eqref{eq:lem_model_estimation_err} the bounds on $(A)$ and $(B)$ concludes the proof. 
\end{proof}

\begin{proof}
    Let $\nabhat_t = \frac{1}{N}\sum_{i\in\sbrac{N}}{\nabla f_i(\hat{x}_t^i)}$. From the $\beta$-smoothness of the objective, 
    \begin{align}\label{eq:one_step_improvement}
        \bbE[f(x_{t+1}) - f(x_t)] &\leq -\eta\bbE[\hat{g}_t^\top\nab_t] + \frac{\beta\eta^2}{2}\bbE\norm{\hat{g}_t}^2 \nonumber \\ &= - \eta\bbE[\nabhat_t^\top\nab_t] + \frac{\beta\eta^2}{2}\bbE\norm{\hat{g}_t}^2 \nonumber \\ &= - \eta\bbE\norm{\nab_t}^2 + \underbrace{\eta\bbE[\nab_t^\top(\nab_t - \nabhat_t)]}_{=(A)} + \frac{\beta\eta^2}{2}\bbE\norm{\hat{g}_t}^2 \; ,
    \end{align}
    where the first equality follows from the law of total expectation, and the second equality from the linearity of expectation. 

    \paragraph{Bounding $(A)$: } Using the inequality $a^\top b\leq \frac{1}{2}\norm{a}^2 + \frac{1}{2}\norm{b}^2$, we get that
    \begin{equation*}
        \eta\bbE[\nab_t^\top(\nab_t - \nabhat_t)] \leq \frac{\eta}{2}\bbE\norm{\nab_t}^2 + \frac{\eta}{2}\bbE\norm{\nab_t - \nabhat_t}^2\; . 
    \end{equation*}
    Focusing on the second term in the right-hand side, we have:
    \begin{align*}
        \bbE\norm{\nab_t - \nabhat_t}^2 &= \bbE\bnorm{\frac{1}{N}\sum_{i=1}^{N}{\brac{\nabla f_i(x_t) - \nabla f_i(\hat{x}_t^i)}}}^2 \leq \frac{1}{N}\sum_{i=1}^{N}{\bbE\norm{\nabla f_i(x_t) - \nabla f_i(\hat{x}_t^i)}^2} \leq \frac{\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2}\; ,
    \end{align*}
    where in the first inequality we used Lemma~\ref{lem:technical_norm_of_sum_to_sum_of_norms}, and the second inequality follows from the $\beta$-smoothness of each $f_i$. Plugging back this bound,
    \begin{equation*}
        \eta\bbE[\nab_t^\top(\nab_t - \nabhat_t)] \leq \frac{\eta}{2}\bbE\norm{\nab_t}^2 + \frac{\beta^2\eta}{2N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2}\; .
    \end{equation*}

    Using Lemma~\ref{lem:second_moment_bound} and the bound on $(A)$, we get from Eq.~\eqref{eq:one_step_improvement} that
    \begin{align}
        \bbE[f(x_{t+1}) - f(x_t)] &\leq -\frac{\eta}{2}\bbE\norm{\nab_t}^2 +  \frac{\beta^2\eta}{2N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2} + \frac{\beta\eta^2}{2}\brac{\tilde{\sigma}^2 + 4\gamma\bbE\norm{\nab_t}^2 + \frac{2\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2}} \nonumber \\ &= \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2}\bbE\norm{\nab_t}^2 + \frac{\beta\eta^2\tilde{\sigma}^2}{2} + \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}\cdot\frac{2\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2} \nonumber \; .
    \end{align}
    Note that we can bound $2\beta^2\bbE\norm{\hat{x}_t^i - x_t}^2$ for every $i\in\sbrac{N}$ using Lemma~\ref{lem:model_estimation_error}. Since the bound in Lemma~\ref{lem:model_estimation_error} is independent of the client's identity $i$, it also holds for the average over the clients, i.e.,
    \begin{equation*}
        \frac{2\beta^2}{N}\sum_{i=1}^{N}{\bbE\norm{\hat{x}_t^i - x_t}^2} \leq \sum_{k=1}^{t}{k (2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{t}{(2\alpha)^k\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}\; ,
    \end{equation*}
    where $\alpha=\beta^2\omega^2\eta^2\Tcal^2$. Plugging back, we get that
    \begin{align}\label{eq:one_step_improvement_2}
        \bbE[f(x_{t+1}) - f(x_t)] &\leq \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2}\bbE\norm{\nab_t}^2 + \frac{\beta\eta^2\tilde{\sigma}^2}{2} \nonumber \\ &\quad+ \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}\brac{\sum_{k=1}^{t}{k (2\alpha)^k}\tilde{\sigma}^2 + \frac{4\gamma}{\Tcal}\sum_{k=1}^{t}{(2\alpha)^k\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}} \nonumber \\ &= \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2}\bbE\norm{\nab_t}^2 + \brac{\frac{\beta\eta^2}{2} + \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}\sum_{k=1}^{t}{k(2\alpha)^k}}\tilde{\sigma}^2 \nonumber \\ &\quad+ \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}\frac{4\gamma}{\Tcal}\underbrace{\sum_{k=1}^{t}{(2\alpha)^k\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}}}_{=(B)} \; .
    \end{align}
    Since $2\alpha\leq 1/2 < 1$, we can bound the coefficient of $\tilde{\sigma}^2$ using Lemma~\ref{lem:term_by_term_differentiation} as 
    \begin{equation}\label{eq:linear_times_geomteric_series}
        \sum_{k=1}^{t}{k(2\alpha)^k} \leq \sum_{k=1}^{\infty}{k(2\alpha)^k} = \frac{2\alpha}{(1 - 2\alpha)^2} \leq 8\alpha\; ,
    \end{equation}
    where in the last inequality we used $\frac{1}{(1-2\alpha)^2}\leq 4$. 

    \paragraph{Bounding $(B)$: } To bound $(B)$, we change the summation order. Consider a fixed $\ell\in\naturals$. Note that $(2\alpha)^k$ appears as a coefficient of $\bbE\norm{\nab_\ell}^2$ if and only if $t-k\Tcal\leq \ell\leq t-k$, which is equivalent to $\frac{t-\ell}{\Tcal}\leq k\leq t-\ell$. Therefore, we have 
    \begin{align*}
        \sum_{k=1}^{t}{(2\alpha)^k\sum_{\ell=t-k\Tcal}^{t-k}{\bbE\norm{\nab_\ell}^2}} &= \sum_{\ell=0}^{t-1}{\brac{\sum_{k=\ceil{\frac{t-\ell}{\Tcal}}}^{t-\ell}{(2\alpha)^k}}\bbE\norm{\nab_\ell}^2} \\ &\leq \sum_{\ell=0}^{t-1}{\brac{\sum_{k=\ceil{\frac{t-\ell}{\Tcal}}}^{\infty}{(2\alpha)^k}}\bbE\norm{\nab_\ell}^2} \\ &= \frac{1}{1-2\alpha}\sum_{\ell=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-\ell}{\Tcal}}}\bbE\norm{\nab_{\ell}}^2}
    \end{align*}
    Plugging back to Eq.~\eqref{eq:one_step_improvement_2} gives
    \begin{align}
        \bbE[f(x_{t+1}) - f(x_t)] &\leq \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2}\bbE\norm{\nab_t}^2 + \brac{\frac{\beta\eta^2}{2} + \brac{2\eta + 4\beta\eta^2}\alpha}\tilde{\sigma}^2 \nonumber \\ &\quad+ \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}\frac{4\gamma}{(1-2\alpha)\Tcal}\sum_{k=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-k}{\Tcal}}}\bbE\norm{\nab_k}^2} \nonumber \; .
    \end{align}
    Summing over $t=0,\ldots,T-1$, we obtain
    \begin{align}\label{eq:sum_over_T_err}
        \bbE[f(x_{T}) - f(x_0)] = \sum_{t=0}^{T-1}{\bbE[f(x_{t+1}) - f(x_t)]} &\leq \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2} + \brac{\frac{\beta\eta^2}{2} + \brac{2\eta + 4\beta\eta^2}\alpha} T\tilde{\sigma}^2 \nonumber \\ &\quad+ \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}\frac{4\gamma}{(1-2\alpha)\Tcal}\underbrace{\sum_{t=0}^{T-1}{\sum_{k=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-k}{\Tcal}}}\bbE\norm{\nab_k}^2}}}_{=(C)}\; .
    \end{align}
    Focusing on $(C)$, we can change the outer summation bounds as 
    \begin{equation*}
        \sum_{t=0}^{T-1}{\sum_{k=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-k}{\Tcal}}}\bbE\norm{\nab_k}^2}} = \sum_{t=1}^{T-1}{\sum_{k=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-k}{\Tcal}}}\bbE\norm{\nab_k}^2}} \leq \sum_{t=1}^{T}{\sum_{k=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-k}{\Tcal}}}\bbE\norm{\nab_k}^2}}\; .
    \end{equation*}
    Now, we can bound the right-hand side using Lemma~\ref{lem:double_sum_of_weighted_grads_to_single_sum} with $a=2\alpha<1$ and $x_k = \bbE\norm{\nab_k}^2\geq 0$ to get that
    \begin{equation*}
        \sum_{t=1}^{T}{\sum_{k=0}^{t-1}{(2\alpha)^{\ceil{\frac{t-k}{\Tcal}}}\bbE\norm{\nab_k}^2}} \leq \Tcal\frac{2\alpha}{1-2\alpha}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2}\; .
    \end{equation*}
    Plugging this bound back to Eq.~\eqref{eq:sum_over_T_err} and using the result in Eq.~\eqref{eq:linear_times_geomteric_series} to bound $2\alpha/(1-2\alpha)^2$ by $8\alpha$ gives
    \begin{align*}
        \bbE[f(x_T) - f(x_0)] &\leq \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2} + \brac{\frac{\beta\eta^2}{2} + \brac{2\eta + 4\beta\eta^2}\alpha} T\tilde{\sigma}^2 \\ &\quad+ \brac{\frac{\eta}{4} + \frac{\beta\eta^2}{2}}4\gamma\frac{2\alpha}{(1-2\alpha)^2}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2} \\ &\leq \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2+4\gamma\brac{2\eta + 4\beta\eta^2}\alpha}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2} + \brac{\frac{\beta\eta^2}{2} + \brac{2\eta + 4\beta\eta^2}\alpha} T\tilde{\sigma}^2
    \end{align*}
    Substituting $\alpha=\beta^2\omega^2\eta^2\Tcal^2$, we get that $(2\eta + 4\beta\eta^2)\alpha = 2\omega^2\Tcal^2\beta^2\eta^3 + 4\omega^2\Tcal^2\beta^3\eta^4$. Hence, 
    \begin{align*}
        \bbE[f(x_T) - f(x_0)] &\leq \brac{-\frac{\eta}{2} + 2\gamma\beta\eta^2+8\gamma\omega^2\Tcal^2\beta^2\eta^3 + 16\gamma\omega^2\Tcal^2\beta^3\eta^4}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2} \\ &\quad+ \brac{\frac{\beta\eta^2}{2} + 2\omega^2\Tcal^2\beta^2\eta^3 + 4\omega^2\Tcal^2\beta^3\eta^4} T\tilde{\sigma}^2\; .
    \end{align*}
    Since $\eta\leq \frac{1}{12\gamma\beta\max\cbrac{\omega\Tcal, 1}}\leq \frac{1}{6\beta\max\cbrac{\omega\Tcal, 1}}$, we can now bound the coefficient of $\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2}$ using Lemma~\ref{lem:sum_of_grads_coeff_bound} and the coefficient of $T\tilde{\sigma}^2$ using Lemma~\ref{lem:sigma_tilde_coeff_bound}, both with $\theta=\max\cbrac{\omega\Tcal, 1}$. We get
    \begin{align*}
        \bbE[f(x_{T}) - f(x_0)] &\leq -\frac{\eta}{4}\sum_{t=0}^{T-1}{\bbE\norm{\nab_t}^2} + \beta\theta\eta^2 T\tilde{\sigma}^2\; .
    \end{align*}
    Rearranging terms and multiplying by $4/\eta T$ gives
    \begin{align*}
        \bbE\sbrac{\frac{1}{T}\sum_{t=0}^{T-1}{\norm{\nab_t}^2}} &\leq \frac{4\bbE[f(x_0) - f(x_T)]}{\eta T} + 4\beta\theta\eta \tilde{\sigma}^2 \leq \frac{4M}{\eta T} + 4\beta\theta\eta \tilde{\sigma}^2 \; ,
    \end{align*}
    where $M\coloneqq f(x_0) - f^*$ and the last inequality follows from $\bbE[f(x_T)]\geq f^*$. Finally, there are two cases for $\eta$, which we explicitly consider.

    
    \textbf{Case $\sqrt{\frac{M}{\beta\theta T\tilde{\sigma}^2}}\leq \frac{1}{12\gamma\beta\theta}$: } Substituting the value of $\eta=\sqrt{\frac{M}{\beta\theta T\tilde{\sigma}^2}}$ gives
    \begin{align*}
        \bbE\sbrac{\frac{1}{T}\sum_{t=0}^{T-1}{\norm{\nab_t}^2}} \leq 8\sqrt{\frac{M\beta\theta\tilde{\sigma}^2}{T}}\; .
    \end{align*}

    
    \textbf{Case $\frac{1}{12\gamma\beta\theta}< \sqrt{\frac{M}{\beta\theta T\tilde{\sigma}^2}}$: } Here $\eta = \frac{1}{12\gamma\beta\theta}$. Plugging the value of $\eta$ in the first term and bounding $\eta$ above by $\sqrt{\frac{M}{\beta\theta T\tilde{\sigma}^2}}$ in the second term gives
    \begin{align*}
        \bbE\sbrac{\frac{1}{T}\sum_{t=0}^{T-1}{\norm{\nab_t}^2}} \leq \frac{48\gamma M\beta\theta}{T} + 4\sqrt{\frac{M\beta\theta\tilde{\sigma}^2}{T}} \; .
    \end{align*}

    For both cases we have, 
    \begin{align*}
        \bbE\sbrac{\frac{1}{T}\sum_{t=0}^{T-1}{\norm{\nab_t}^2}} \leq 8\sqrt{\frac{M\beta\theta\tilde{\sigma}^2}{T}} + \frac{48\gamma M\beta\theta}{T}\; ,
    \end{align*}
    which concludes the proof.

\end{proof}

